Wireless Connectivity of a Ground-and-Air Sensor Network

This paper shows that, when considering outdoor scenarios and wireless communications using the IEEE 802.11 protocol with dipole antennas, the ground reflection is a significant propagation mechanism. This way, the Two-Ray model for this environment allows predicting, with some accuracy, the received signal power. This study is relevant for the application in the communication between overflying Unmanned Aerial Vehicles (UAVs) and ground sensors. In the proposed Wireless Sensor Network (WSN) scenario, the UAVs must receive information from the environment, which is collected by sensors positioned on the ground, and need to maintain connectivity between them and the base station, in order to maintain the quality of service, while moving through the environment.

==> 31_theproblem.tex <==
\section{The Problem}
Environmental monitoring often cannot be effectively done only through image analysis (taken from overflights), but requires the periodic collection of  data from hundreds or even thousands of sensors on the ground or close to the ground, such as at tree crops. These sensors may be used to monitor factor, such as humidity, temperature, slight tremors or slight displacements of soil that are hardly noticeable by humans. In this cases, the best approach is to spread  sensor nodes - hundreds or thousands of them - and use UAVs to periodically visit the nodes and collect this data from the sensor nodes.

However, since there might be too many of such sensor nodes on the ground, a swarm of UAVs coordinating their itineraries should be used. Moreover, there might be several sensor nodes that have been put at places, among two large stones or under a bush of trees, where a UAV visit and/or the vertical wireless transmission of data is hindered. Therefore, the sensor nodes have to build a mesh network and route each node's sensor data towards the directions of the mesh nodes that are being visited.

But this highly dynamic routing and collection of data among mesh sensor nodes and a fleet of UAVs poses several challenges that are due to the inherent mobility of the UAVs, such as wireless interference (e.g. between the vertical and the horizontal data transmissions) and other propagation problems inherent to the wireless environment. Therefore the goal of this project is to predict the wireless communication channel between the sensors and the UAVs, more specifically our interest is to calculate the Received Signal Strength (RSS) based on transmitter power, type of antenna and polarization used, considering a realistic soil and using the 802.11 modulation scheme, often known as “wi-fi” at frequency of 2.412 Ghz (channel 1).

\begin{figure}[ht]
    \includegraphics[width=8cm]{figs/EspacoAeromodelismo-Aterro3.jpg}
    \centering
    \caption{Propagation test environment.}
    \label{fig:Aterro}
\end{figure}


==> 4_wireless.tex <==
\section{Wireless Connectivity}

In terms of the wireless environment, we simulated the propagation of RF waves between two drones using a classical ray-tracing model. The proposed outdoor scenario does not provide multiple rays being reflected or diffracted. Hence, two rays were considered in the calculations, the direct ray and the one reflected by the ground, which reduces our model to the deterministic two-ray model \cite{Molisch2004}.

In order to validate the model, experimental measures were done in an aeromodelling field at Aterro do Flamengo. The dimensions of this field, in meters, are shown in Fig. \ref{fig:Aterro}.

\begin{figure}[ht]
    \includegraphics[width=8cm]{figs/EspacoAeromodelismo-Aterro3.jpg}
    \centering
    \caption{Propagation test environment.}
    \label{fig:Aterro}
\end{figure}

In addition, the impact of the antennas radiation patterns was also considered. This way, the drone antennas were considered as being half-wave dipoles, which present omnidirectional planes of propagation. Both polarization planes were considered: vertical and horizontal. Table \ref{tab:parameters} shows the parameters used in the wireless channel simulations \cite{Ometov2019}.

\begin{table}[ht]
\begin{center}
\caption{Parameters of the Wireless Channel Simulations}
\label{tab:parameters}
\vspace{0.5cm}
\begin{tabular}{c c c}

\toprule[1.0pt]
Parameter & Description & Value\\
\midrule[1.0pt]
$P_{TX}$ & Transmitter power & 10 dBm \\
$L_{T}$ & ESP32 transmitter loss & 1.5 dB \\
$L_{R}$ & Adalm Pluto receiver loss & 2.5 dB \\
$L_{C}$ & Cable loss & 0.6 dB \\
$L_{D}$ & Resistive divider loss & 7.1 dB \\
$G_{max}$ & Maximum antenna gain & 1.97 dB \\
$S_{r}$ & ESP32 receiver sensitivity  & --85 dBm \\
$f$ & Signal frequecy & 2.412 GHz\\
$d$ & Link horizontal distance & 0 -- 50 m \\
\midrule[1.0pt]\\

\end{tabular}
\end{center}
\end{table}

==> 5_1_Ray_Tracing.tex <==
\section{Ray Tracing}
Wireless propagation channels have the disadvantage in relation to guided channels that the signal is subject to multipath, so the electromagnetic waves can reach the receiver through different paths, being able to be reflected, refracted or diffracted along the way.
In the simplest case, the wave propagates in free space, without encountering any obstacles, so there is no reflection or absorption of energy by objects in the vicinity of the antenna, in this case, the attenuation caused by the free space can be defined by the following well-known equation:

\begin{equation}
FSL=32.45+20log(D_{Km})+20log(f_{MHz})
\end{equation}

However, only a direct path between the base station and the transmitting antenna is hardly the only propagation mechanism, so the free space loss model alone becomes, in most situations, inaccurate for describing the signal propagation.

Then, is make use of more sophisticated techniques, for instance, ray tracing, which  
is a method to determine the rays that leave a transmitter and arrive at the receiver, considering a finite number of reflectors and their dielectric properties. A feature of this model is that is simulated the inverse path of the wave, thus the receiver acts as the source of the rays and the transmitter as the receiver, in this way, in the modeling, the ground station receives the waves transmitted by the drone.

The two-ray model is a particularization of ray tracing, considering only two paths: a direct line of sight path and a ground reflection. Thus, the energy that arrives at the receiving antenna comes from different paths, where each incident wave arrives from different directions and at different times (delay), therefore traveling different paths, they have different phases. In turn, when arriving at the receiver, the waves can add constructively or destructively depending on their wave phases.

Reflection occurs when the propagating electromagnetic wave hits an obstacle with dimensions much larger than its wavelength. The interest is to calculate the intensity of the wave reflected to the environment and that reaches the receiver, defined through the Fresnel reflection coefficient, given by the formulas:
\begin{equation}
    \Gamma_\parallel= \frac{E_r}{E_i}=\frac{-\varepsilon_g sen\theta_i+\sqrt{\varepsilon_g-cos\theta_i^2}}{\varepsilon_g sen\theta_i+\sqrt{\varepsilon_g-cos\theta_i^2}}
  \end{equation}
  

  \begin{equation}  
    \Gamma_\perp= \frac{E_r}{E_i}= \frac{sen\theta_i-\sqrt{\varepsilon_g-cos\theta_i^2}}{ sen\theta_i+\sqrt{\varepsilon_g-cos\theta_i^2}}
\end{equation}

And which depend on the polarization (vertical and horizontal, respectively) and the angle of incidence  of the wave with the ground, the complex relative permittivity of the soil in relation to that of the air, considering the conductivity of the soil, given by:

\begin{equation}
    \varepsilon_g=\varepsilon_r-j\frac{\sigma}{\omega\varepsilon_0}=\varepsilon_r-j60\sigma\lambda_0
\end{equation}


\begin{table}[ht]
\begin{center}
\caption{Parameters of the Wireless Channel Simulations}
\label{tab:parameters}
\vspace{0.5cm}
\begin{tabular}{c c c}

\toprule[1.0pt]
Parameter & Description & Value\\
\midrule[1.0pt]
$\varepsilon_r$ & relative permittivity grass & 42 \\
$\varepsilon_r$ & relative permittivity concrete & 1.7 \\
$\sigma$ & conductivity soil & 0 $(\Omega m)^-1$ \\

\midrule[1.0pt]\\

\end{tabular}
\end{center}
\end{table}

Moreover, in the simulation, the flat Earth propagation model is admitted, where the divergence factor (D) that quantifies the effect of the divergence of the wave reflected on the spherical surface of the Earth is equal to 1. This consideration can be made since the antennas are small in relation to the radius of the earth and that the distance between them is much greater than the order of size of their heights.

Furthermore, another effect to consider is the diffuse reflection of rays on rough ground. The scattering coefficient that quantifies the degree of scattering of rays is given by:

    % rho_s = exp(-0.5.*(delta_fase.^2));
\begin{equation}
    \rho_s=e^{-0.5\Delta\phi^2}
\end{equation}

With these considerations in mind, we arrive at the mathematical formulation of the two-ray model:
\begin{equation}
P_r=P_t\left[\frac{\lambda}{4\pi}\right]^2\left[\frac{\sqrt{G_l}}{l}+\frac{\rho_s D\Gamma\sqrt{G_r}e^{-j\Delta\phi}}{x+x'}\right]^2
\end{equation}

Where is the phase difference of the two received rays.

\begin{figure}[ht]
    \includegraphics[width=8cm]{figs/2raymodel.png}
    \centering
    \caption{Schematic of 2 ray model}
    \label{fig:Schematic of 2 ray model}
\end{figure}


==> 8_Machado_Couto.tex <==
\section{description of IEEE 802.11 modulations (Machado)}

\subsection {Differences between 802.11 patterns} 

The process of transmitting information in various 802.11 standards is carried out by two techniques: Direct Sequence Spread-Spectrum (DSSS) and Orthogonal Frequency-Division Multiplexing (OFDM).

In this context, 802.11g uses DSSS, as well as the 802.11b, and OFDM, similarly to 802.11n. However, there are differences between these techniques in each standard. For example, the specifications of bandwidth, data rate and modulations used in the signal transmitted, such as BPSK, QPSK, 16-QAM, 64-QAM, varies for each application. 

Furthermore, they all specify a spectral mask that filters the modulated signal to the limit bandwidth of channel to avoid interference and, hence, loss of information. 


\begin{figure}[!ht]
    \includegraphics[width=5cm]{figs/MACHADO1.jpeg}
    \centering
    \caption{Spectral Masks of 802.11b/g/n, with their specific characteristic \cite{Interference}}
    \label{fig:WLAN Channels}
\end{figure}



\subsection {DSSS}

Direct Sequence Spread-Spectrum is a technique that implements the extension of the original signal's bandwidth to reduce interference on the information. 

First, it introduces a binary pseudorandom sequence generator to spreading the signal, in which only the receiver knows how to decrypt. Then, the DSSS signal is modulated and passes through the spectral masking filter to limit it's power. At the receiver, the signal will again pass through a matched filter to inhibit part of the noise introduced by the channel and will be demodulated. Following, another pseudorandom sequence generator will add the same code to despreading  the signal. Therefore, the decoding of the signal is processed, since the added noise has been attenuated due to scattering.

\begin{figure}[!ht]
    \includegraphics[width=10cm]{figs/MACHADO2.jpeg}
    \centering
    \caption{Diagram of DSSS in frequency}
    \label{fig:Diagram of DSSS in frequency}
\end{figure}



In the following figure, it is represented the aspect of signal over time.
\begin{figure}[!ht]
    \includegraphics[width=5cm]{figs/MACHADO3.jpeg}
    \centering
    \caption{Signal processing at receiver over time \cite{Performance}}
    \label{fig:Signal processing at receiver over time}
\end{figure}

Acording with Communications Systems \cite{Communication}, mathematically:

The input signal is:
\begin{equation*}
v(t)=\sum_{n=-\infty}^{\infty} a_n g_T(t-nT_b)
\end{equation*}

In which 
\begin{equation*}
a_n=\pm1, -\infty<n<\infty
\end{equation*}

The generated pseudorandom sequence is given by:
\begin{equation*}
c(t)=\sum_{n=-\infty}^{\infty} c_nP(t-T_C)
\end{equation*}

With P(t) called chip and c(t) = \pm 1.
The generated DSSS signal has the following equation:
\begin{equation*}
u(t)=A_c v(t)c(t)cos(2\pi f_ct)
\end{equation*}

Considering the channel noise:
\begin{equation*}
r(t)=A_c v(t)c(t)cos(2\pi f_ct)+i(t)
\end{equation*}

Despreading:
\begin{equation*}
c(t)r(t)=A_c v(t)cos(2\pif_ct)+i(t)c(t)
\end{equation*}

In the case in which the noise is sinusoidal, that is:
\begin{equation*}
i(t)=A_I cos(2\pi f_I t)
\end{equation*}

The power's interference is:
\begin{equation*}
I_0R_b=P_IR/W=\frac{P_I}{W/R}=\frac{P_I}{L_c}
\end{equation*}


Hence, it is tangible to obtain the quantity of power for which interference has been added, as long as the channel and noise characteristics are known.

\subsection {OFDM} 

The OFDM technique transmits data through K subcarriers, which K is defined by the standard 802.11 implemented, modulated in QAM or PSK \cite{tecnica}, with a transmission rate K times lower than the original. This kind of technique in which narrow a signal width helps in frequency selectivity, that is, the subcarrier response to the channel is constant in the spectrum domain, what significantly reduces the use of more complex equipment \cite{tecnica}.

\begin{figure}[!ht]
    \includegraphics[width=7cm]{figs/MACHADO4.jpeg}
    \centering
    \caption{Difference between Conventional multicarrier technique and Orthogonal multicarrier modulation technique \cite{Power}}
    \label{fig:Signal processing in time at receiver}
\end{figure}

The original signal is divided into bit blocks by the serial-parallel converter and they are modulated in according with the 802.11 standard, which can be BSPK, QPSK, 16-QAM, 64-QAM \cite{tecnica}. To avoid interference between spectra, the subcarriers are ranged at zero crossing points, that is, they are orthogonal, meaning that:

\begin{equation*}
\int_{0}^{T} cos(2 \pi f_k+\phi_k)cos(2 \pi f_j+\phi_j)dt=0
\end{equation*}

Then, these subsymbols pass through the IFFT to be filtered and a guard interval is added to prevent inter-symbol interference (ISI). Thus, the total duration time of OFDM symbol will be given by $T_s+T_g.$

\begin{figure}[!ht]
    \includegraphics[width=5cm]{figs/MACHADO5.jpeg}
    \centering
    \caption{Power Spectrum Density of signal after modulated in OFDM (black), mask spectrum filter (red) and received with a noise added (green). \cite{Peak}}
    \label{fig:Power Spectrum Density of signal after modulated in OFDM (black), passed by a mask spectrum filter and received with a noise added}
\end{figure}

After the transmission of the channel, the reverse process occurs. First, the guard intervals are removed and FFT is applied for each subcarrier. Then, the inverse mapping transform a OFDM signal in a bit block. In the end, a series-parallel converter convert these blocks into the original information code.

\begin{figure}[!ht]
    \includegraphics[width=10cm]{figs/MACHADO6.jpeg}
    \centering
    \caption{Block diagram of OFDM \cite{Communication} }
    \label{fig:Signal processing in time at receiver}
\end{figure}

==> 9_Santiago.tex <==
\section{OMNeT++ Implementation for the Two-Ray Ground-Reflection Model}

\subsection{OMNeT++}
OMNeT++ is discrete-time event simulator, which is extensible and contains an open source library available for free use, structured in object-oriented programming, more specifically C++. It's main purpose is to build network simulations, implementing physical models and other network layers protocols. The main focus here will be the discussion about the implementation already offered in the INET library, and it/s comparison to the new version implemented in this research work.  

\subsection{INET version for the Two-Ray Model}

The version presented at OMNeT++ for this propagation model consists only in the flat earth approximation for the terrain in it's simulation. The conditions presented in this code only are concerned only in the criteria for Free Space Path Loss or the more generic Flat Earth Model. The code in itself calculates the respective altitudes and relative distances between the transmitter, the receiver and the reflection point at the soil from the configurations inserted by the user in the .ini file, and calculates the wavelength of a narrow band signal from it's speed of propagation and it's center frequency. In it's more general presentation (and with divergence factor considered to be 1, in the Flat Ground case), the program realizes the simulation with the well known result for attenuation:
$$\frac{h_{t}^2 h_{r}^2}{d^4}$$
Where $h_{t}$ and $h_{r}$ are the transmitter and the receiver altitudes, respectively, and $d$ is the distance between the antennas. 

\subsection{New version for the Two-Ray Model}
The new project developed has some significant alterations aiming for more precise and realistic simulations. The first one is the analysis of the conditions for decision between the Flat Earth and Spherical Earth models for the Two-Ray propagation, based in the comparison of the distance between the antennas and the value obtained by calculating the radium horizon (realized by taking the highest altitude between that of the transmitter and the receiver).
Since the relative distances and heights used in the  practices conducted in field attend the sufficient criteria for Flat Earth approximation, the Spherical Earth will not be discussed in the present article.

Besides that, some alterations were included in the computation of the reflection coefficient, now a complex value (since now the conductivity of the soil was taken into account). The relative permissiveness of air and soil were adjusted to be respectively 1 and 15, values obtained from the simulations realized in MATLAB. the third and final significant change is now the possibility for use both horizontal and vertical polarization, predominantly in dipole antenna type (which had it's code edited as well, to include more realistic irradiation diagrams and display of it's directional lobes). This change allows to switch between both possible computations for the complex valued reflection coefficient. 

The computation of the propagation by the Flat earth model is in itself similar, it's main difference being the calculus of the reflection coefficient depending on the polarization of the antennas (Gamma Parallel of Orthogonal) and the computation of the relative distances to the reflection point for the equating of the interference term.
Lastly, the calculus of the wavelength were left identical to those of the code provided in the INET library, using a narrow band signal, as well as the obtaining of the heights of each antenna. 

\subsection{Comparison between the old and new codes for Two-Ray Ground Reflection model}





\subsection{Configuring done in the .ini file}
In OMNeT++, an initialization file (.ini) is a type of archive that carries all the configurations that will be implemented in the network simulation. In this subsection, the most relevant type of parameters used and its values will be presented, so that the reader can eventually reproduce the simulation.


Bibliography: 
(Se tiver ok coloco no final nos moldes de artigo de cientifico)
Rappaport, Theodore: Wireless Communications - Principles and Practice, 2nd edition, 2002
 Jakes, William C.: "Microwave Mobile Communications", 1974
